Generalized Decomposition Priors on R2

The adoption of continuous shrinkage priors in high-dimensional linear models has gained widespread attention due to their practical and theoretical advantages. Among them, the R2D2 prior has gained popularity for its intuitive specification of the proportion of explained variance (R2) and its theoretically grounded properties. The R2D2 prior allocates variance among regression terms through a Dirichlet decomposition. However, this approach inherently limits the dependency structure among variance components to the negative dependence modeled by the Dirichlet distribution, which is fully determined by the mean. This limitation hinders the prior's ability to capture more nuanced or positive dependency patterns that may arise in real-world data. To address this, we propose the Generalized Decomposition R2 (GDR2) prior, which replaces the Dirichlet decomposition with the more flexible Logistic-Normal distribution and its variants. By allowing richer dependency structures, the GDR2 prior accommodates more realistic and adaptable competition among variance components, enhancing the expressiveness and applicability of R2-based priors in practice. Through simulations and real-world benchmarks, we demonstrate that the GDR2 prior improves out-of-sample predictive performance and parameter recovery compared to the R2D2 prior. Our framework bridges the gap between flexibility in variance decomposition and practical implementation, advancing the utility of shrinkage priors in complex regression settings.

==> ims-template/archive.tex <==
\subsubsection{Extensions and more}


\textit{Normalization of random variables}

\PB{Paul Buerkner: did we make a decision on in how much detail we want to introduce other distritbutions that we will later on choose to ignore?
}

The most immediate way to produce random vectors that belong to the simplex is by considering random variables $Z_1, ..., Z_p$, where $Z_k \in \mathbb{R}$ (which naturally implies that the random vector $(Z_1,..., Z_p) \in \mathbb{R}^p$), and transforming them into the simplex via a transformation $\Psi: \mathbb{R}^p \to \mathcal{S}^p$. The form of $\Psi$ can vary enormously. For instance, the user can consider the following transformation, which is highly intuitive, $\phi_k = \frac{Z_k}{ \sum_{k=1}^p Z_k}$ or $\phi_k = \frac{e^{Z_k}}{ \sum_{k=1}^p e^{Z_k}}$. Although using this method is a natural and simple way to follow, we might find difficulties in finding the proper Jacobian adjustments and analytic expressions for the resulting densities, a sufficiently flexible function $\Psi$ that entails our objectives and represents no computational problems and one might not have a real idea over the properties that the distribution of $\phi$ will have. Due to this reasons, we consider that one should make use of distributions that have been studied in depth such as the ones presented below. 

\textit{Multiplicative LN}


\textit{Flexible Dirichlet Distribution}


\textit{Nielsen's Simplex Distribution}


The standard derivation of the Dirichlet distribution involves producing a random vector $\phi \in \mathcal{S}^p$ by generating $p$ independent gamma random variables $Z_i \sim \gammadist(\alpha_i,\beta)$ with a common scale parameter $\beta$ and then normalizing them by their sum. \cite{simplex_nielsen} introduce a more general class of simplex distributions by considering the use of Generalized Inverse Gaussian (GIG) \citep{RobertGIG} instead. The Dirichlet distribution can be obtained as a special case, since gamma distributions are a subclass of the GIG distributions. 

We will say that a random variable $Z$ follows a Generalized Inverse Gaussian distribution and we denote it by $Z \sim  \gigdist(\alpha, \chi, \psi )$ if its density with respect to the Lebesgue measure has the form
 
\begin{align}
    p(z | \alpha, \chi, \psi) = \frac{\left( \chi \psi \right)^{\alpha/2}}{2 K_\alpha \left(  \sqrt{\chi \psi}  \right) } z^{\alpha-1} e^{\left(  - \chi z^{-1}  + \psi z \right)/2},
\end{align}

where $K_\alpha$ is a Bessel function and $z>0, \chi, \psi >0 , \alpha \in \mathbb{R}$ \citep{simplex_nielsen, RobertGIG}. Furthermore, let $Z_1,..., Z_p$ be independent and distributed according to $Z_k \sim \gigdist(\alpha_k, \chi_k, \psi)$, i.e they have a common $\psi$, and let $Z_+= \sum_{k=1}^p Z_i$. Let $\alpha_k=-1/2$ for $k=1,..., p$ which implies that $Z_k$ has an inverse Gaussian distribution and let $\phi_k = \frac{ Z_k}{ Z_+}$, then the density of $\phi= (\phi_1,..., \phi_k)$ with respect to the Lebesgue measure has the form 
%------------------
\begin{align}
\label{eq:simplex_nielsen}
p(\phi | \mu, \lambda) = \left(\frac{\lambda}{ 2\pi } \right)^{(p-1)/2} \left( \prod_{k =1} \phi_k\right)^{-3/2} e^{\lambda t( \phi; \mu) },
\end{align}
%------------------
where $t( \phi; \mu) \coloneqq  -1/2  \left( \prod_{k =1} \mu_k \right)^{-2/(p-1)} Q(\phi;\mu), \mu_k= \frac{ \sqrt{\chi_k} }{ \sum_{k=1}^p \sqrt{\chi_k} }$ and $Q(\phi;\mu) \coloneqq \sum_{k=1}^p \frac{  \mu_k^2}{ \phi_k} -1 $ \citep{simplex_nielsen}. We will denote the distribution presented in \eqref{eq:simplex_nielsen} as the \textbf{put a name} distribution and  $S_p(\mu, \lambda)$ and we shall refer to $\mu$ and $\lambda$ as the position and precision parameters, respectively. It is noteworthy to mention that \cite{simplex_nielsen} provide a more general distribution for arbitrary $\alpha$ and $\psi_i$ but we are specifically interested in the case presented, due to the properties we discuss shortly. 

The conditional distributions and the marginal distributions of $S_p( \cdot, \cdot)$ are of the same class \citep{simplex_nielsen}. Let $\phi^{I}=(\phi_k)_{k\in I}$ and $\phi^{\bar{I}}=(\phi_k)_{k \not\in I}$ where $I \subset \{ 1,..., k\}$ and let $\mu^{I}$ and $\mu^{\bar{I}}$ be defined in a similar way. Then the marginal distribution of $\tilde{\phi} \coloneqq ( \phi^{I}, 1- \sum_{k \not \in I} \phi_k ) $ is given by 

\begin{align}
\label{eq:simplex_nielsen_marginal}
     \tilde{\phi} \sim S_{|I|} \left(  \tilde{\mu},  \lambda \left( \prod_{k=1}^p \mu_k \right)^{-2/(p-1)} \left\lbrace\left(\prod_{k \in I}^p \mu_k  \right) \left( 1- \sum_{k \not\in I} \mu_k \right) \right\rbrace^{-2/|I|}   \right), 
\end{align}

where $\tilde{\mu}\coloneqq ( \mu^{I}, 1- \sum_{k \not \in I} \mu_k ) $. The main difference between the Dirichlet distribution and the $S_-$ distribution consists in how the Dirichlet distribution presents the subcompositional independence property, whereas the $S_-$ does not \citep{simplex_nielsen}. Nonetheless the $S_-$ distribution is able to acquire a special form of amalgamation, while the LN does not possess an invariant system under it. In this sense, the $S_-$ is an intermediate step between the Dirichlet and the LN distributions. 

% \TODO{ignore this paragraph}
% There have been efforts to propose alternative distributions for random vectors that live in the simplex. Some of them \textbf{cite} are able to express the  Dirichlet distribution as a particular case. For instance, it is well known that the Dirichlet distribution is not able to \textbf{insert here}, therefore \textbf{cite} have proposed the \textbf{insert here}. In this section we present some distributions that also seem sensible to explore due to their properties. 


% \TODO{Integrate into the text:}

% However, it is in general (or we) consider that the use of these extended distributions is not practical enough and represents theoretical exercises that aim at preserving properties that the Dirichlet distribution has. Additionally, the parameters involved intuitive interpretations, usually presenting a high number of hyperparameters to achieve the proposed objectives. Finally, since the Dirichlet distribution can be formulated as a special case in most of the extended distributions, users might be tempted to represent statistical insights via use of the former, which might imply adding complexity but still using the known tool in the repertoir.  


%---------


A key question is whether or not the arbitrarily selected divisor $\phi_p$ plays an important role in the statistical analysis that can result from using the ALN distribution. \textbf{Aitchison 1986 book cite} shows that resulting inferences are invariant to the choice of the divisor and permutations of the vector $\phi$, i.e the order of the elements of $\phi$ is not relevant. Nonetheless, a way of avoiding the problem of selection is to divide by the geometric mean, a procedure also known as the \textit{centered log-ratio} (clr) transformation \textbf{cite}. If we let $\gm(\phi) \coloneqq \left( \prod_{i=1}^p \phi_k \right)^{1/p}$ represent the geometric mean of $\phi$ then the clr transformation is given by
%--------------------------%
\[ \eta= \clr(\phi) \coloneqq \left(  \log \left( \frac{\phi_{1}}{\gm(\phi)} \right), ...,  \log \left( \frac{\phi_{p-1}}{\gm(\phi)} \right)  \right).   \]
 %--------------------------%
 The disadvantage of this is that the covariance matrix that arises is singular, presenting a need to adapt standard multivariate statistical techniques. Additionally notice that the clr is dependent on which components are included or not in the composition. A key step forward, which might be surprising at first, is to recognize that it is possible to represent elements of the simplex by their coordinates in the simplex with a suitable orthonormal basis \textbf{cite several here}, i.e the simplex can be endowed with a Euclidean structure. \textbf{Cite Egozue 2003} suggest an alternative transformation known as the \textit{isometric log-ratio }(ilr) which avoids both the arbitrariness of the alr and singularity of the clr, but is based on finding an appropriate orthonormal basis that preserved distances between mapped points. A strong disadvantage is that choice of the orthonormal basis for the simplex is not clear and interpretation of the model turns out to be convoluted \textbf{cite}. 

\TODO{Mention we will work with alr. }

During the last decades there has been quite much discussion on which is the proper way of modeling compositional quantities (\textbf{cite cite cite}). We do not aim to provide an answer to which is the best modeling approach, but to make use of the appropriate modeling tools and to introduce their use to shrinkage priors. 





%---------- 19.12.2023
    % Perhaps the most famous Global-Local shrinkage prior is the Horseshoe prior\cite{Horseshoe, HorseshoeProceedings}, which owes its name to the fact that when $\tau=\sigma=1$ and the local scale $\lambda_k$ follows a half-Cauchy prior \citep{GelmanCauchy, PolsonHalfCauchy} , i.e $ \lambda_k \sim C^+(0,1)$, then $\kappa_k \sim \betadist(1/2, 1/2)$.    %----------
    % Figure \textbf{(INSERT FIG} shows the shrinkage profiles (c\textbf{heck name}) for different global local shrinkage priors. In the ideal case noise ($b_k = 0 $) is shrunken strongly towards zero, whereas sufficiently strong signals should remain unaffected., i.e $ \mbe[b_k \given y_i]  \approx y_i$. Mild signals should experience soft and continuous thresholding. 

% Additionally, let the true vector $b$ belong to the class of \textit{nearly-black} vectors $l_0[s_n]=\left \lbrace b \in \mathbb{R}^n: \sum_{i=1}^n \mathbbm{1} \{b_k \neq 0 \}  \leq  s_n \right \rbrace$ for some $s_n$, where $s_n$ is the number of non-zero elements $b$ has (the number of true signals). If $s_n$ is known, then we say that we are under the \textit{non adaptive case} \citep{vanDP2021theoretical}. 


% \subsection{Shrinkage factors and effective number of coefficients}
% \PB{Paul Buerkner: the formulas below are general for GL priors right? Why not introduce them there?
% }

% When performing Bayesian inference, the prior can be seen as a regularizer. This is clearly exemplified when using the Bayesian LASSO or other Bayesian shrinkage priors \citep{bayesianlasso,BayesPenalizedRegSara}, since the posterior modes under these priors correspond to certain frequentist regularizers \citep{DirichletLaplace}. Usual frequentist properties are not precisely equivalent; for instance, the posterior distribution for a continuous random variable is not able to produce exact sparse results, as the latter would require a point mass at zero. When using shrinkage priors, some authors have been able to express the posterior means as shrunken versions of (unshrunken) frequentist estimators \citep{PiironenHorseshoe}, which in practice can lead to a better out-of-sample predictive performance and a decrease in the variance of the point estimators \citep{Ridge}. \textbf{As mentioned before,} several authors have used the concept of \emph{shrinkage factors} to study the amount of shrinkage the prior induces on the regression coefficients towards zero and the effect of the different values of the hyperparameters \citep{Horseshoe, PiironenHorseshoe, BaiHypothesisNB, PolsonHalfCauchy, aguilar_intuitive_2023}. 

% Consider Model \eqref{eqn::linreg} with a prior of the form \eqref{eqn::glprior}, assuming $n \geq p$ and $X$ of full rank, the conditional posterior means of $b$ are given by
% %----------------------------
% \begin{align}
%     \mbe( b | \lambda, \tau, \sigma ) &= (X'X+ \Lambda_b^{-1})^{-1} X' y  \\
%     \nonumber &= \Lambda_b \left(   (X'X)^{-1} +  \Lambda_b \right)^{-1} \hat{b},
% \end{align}
% %----------------------------
% where $\hat{b}$ is the Maximum Likelihood Estimator (MLE). If the predictors are uncorrelated with zero mean and variances $\var(x_i) = \sigma_{x_i}^2$, then $n X' X \approx  n \diag \{ \sigma_{x_1}^2, ...., \sigma_{x_p}^2 \}$ and we have
% %----------------------------
% \begin{align}
%     \mbe( b | \lambda, \tau, \sigma, y  ) &= (X'X+ \Lambda_b^{-1})^{-1} X' y  \\
%     \nonumber &= \Lambda_b \left(   (X'X)^{-1} +  \Lambda_b \right)^{-1} \hat{b}.
% \end{align}
% %----------------------------
% The shrinkage factors have the form
% %----------------------------
% \begin{align}
%     \kappa_k = \frac{1}{1+ n\tau ^2 \sigma_{x_i}^2 \lambda_k^2}.
% \end{align}
% %----------------------------
% % \textbf{Option 2: $\kappa$ with $X= I_n$}

% % Consider Model \ref{eqn::linreg} with a prior of the form \ref{eqn::glprior}, assuming $ X= I_n$, i.e $p=n$ the normal means problem, the conditional posterior means of $b$ are given by
% % %----------------------------
% % \begin{align}
% %     \mbe( b_k | \lambda, \tau, \sigma, y ) &=  (1-\kappa_k) \hat{b}_i.
% % \end{align}
% % %----------------------------
% % where $\hat{b}_i= y_i $ is the Maximum Likelihood Estimator (MLE) and $\kappa_k$ represents the $i$th shrinkage factor with form
% % %----------------------------
% % \begin{align}
% %     \kappa_k &= \frac{1}{ 1+  \lambda_k^2 \tau^2}.
% % \end{align}
% % %----------------------------
% \TODO Possibilities we have:
% \begin{enumerate}
%     \item Fix $\tau$ and consider the distribution as a transformation of $\lambda$. Remembering that $\lambda_k= \phi_k$. This brings problems as the marginals of $\phi$ are not usually known.
%     \item Fix $\phi$ first. Might make sense a priori, since the user could have an idea of a priori proportions. Take $\kappa$ as a transformation of $\tau$. This is what we have done in the R2D2M2 paper.
    
%     \item Consider examples in which we know the marginal of $\phi$. In all cases we have that $\tau \sim \betaprime$. Look for the distribution of the product. This is possible. This would be illustrate the effect that the different distributions on the simplex have on $\kappa$.
%     \item In any case, we can always present numerical examples and compare visually. Plots can take similar forms so how do we select the distribution? 
% \end{enumerate}


% We have used the Dirichlet distribution  $\phi \sim \dirichlet(\alpha)$ and the Logistic Normal distribution $\phi \sim \LN(\mu_\phi, \Sigma_\phi)$ for the decomposition step that involves $\phi$. The specification of the hyperparameters of the R2D2 prior and their effects on posterior estimation have been studied previously\citep{r2d2zhang, aguilar_intuitive_2023}. Thus, we make use of their theoretical guidelines and simulation results to specify the hyperparameters $\{ \mu_{R^2}, \varphi_{R^2}, \alpha \}$.  We set $(\mu_{R^2}, \varphi_{R^2})=(0.5, 1)$ in all simulations to consider non. We discuss how we specify $\alpha$ below.



% Let $\mathcal{F}$ denote a metric of interest and let $\{m_1,...,m_l \} $ be the set of different models under comparison. Let $\mathcal{M}(m_i)$ the value of metric $\mathcal{M}$ for model $m_i$. For a given data set $\mathcal{D}$ denote by $m^*$ the best performing model with respect to the metric $\mathcal{M}$. We define the Delta Metric as $\Delta \mathcal{M}_i, i=1,...,l$ as the difference between the $i$th model and the best model $m^*$ for a fixed given dataset $\mathcal{D}$ \citep{scholz2023prediction}. This is expressed as $\Delta \mathcal{M}_i  \coloneqq \mathcal{M}(m_i) - \mathcal{M}(m^*), \ \ i=1,...,l.$

% The distribution of $\Delta \mathcal{M}_i, i=1,...,l$ across datasets illustrates the performance of the model $m_i$ with respect to the metric $\mathcal{M}$ under the variability of the data generating procedure and explains how model $m_i$ performs in comparison to the other models under different replications. The use of $\Delta \mathcal{M}_i$ stands in contrast with marginally calculating the distribution of the metric  for $m_i$ under different replications, where no consideration is made for its performance in comparison to other models. In practice $\mathcal{M}$ will take the value of the posterior MSE or ELPD on the test set. 
% Coverage properties are studied by inspecting the marginal credibility intervals of the regression coefficients for different sizes $1-\alpha$. Users typically seek insight into the presence or absence of an effect, which in our context is related to treating a coefficient as signal or noise respectively. This is measured by testing the hypothesis $H_0: \theta = 0$ vs $H_0: \theta \neq 0$. Our test statistic is the credibility interval of size $1-\alpha$, which we denote by $I_\alpha$. $H_0$ is rejected at a level $\alpha$ if $0 \not \in I_\alpha$. 

% We can conceptualize hypothesis tests as an outcome of a classification algorithm, where our model functions as the algorithm, producing two output classes: signal or noise. In this context, Type I errors are commonly referred to as False Positive Rates (FPR), while the complement of the Type II error is known as the True Positive Rate (TPR). Adjusting the value of $\alpha$ alters the classification threshold, resulting in a trade-off between FPR and TPR. Therefore, we can evaluate the effectiveness of our classification algorithm using ROC curves \citep{roccurves}. These curves plot TPR against the false positive rate (FPR) at various threshold settings. Ideally, the empirical ROC curve should be concave and nonnegative. A model performing better than random chance should exhibit an ROC curve above the main unit diagonal, i.e., $y=x$, approaching the upper left corner of the unit square. This implies a low FPR and a high TPR \citep{roccurves}.


   %--- Introduce Normal Means 
    % The scenario $y_k | b_k \sim \normal(b_k, 1)$ independently for $k=1,..., K$ is known as the \textit{normal means model} and has been studied profoundly in the last decades \citep{stein1956inadmissibility, Berger1989, Robbins1985AsymptoticallySS, Bernardo2007, vanDP2021theoretical} as it is considered the canonical model in the development of admissibility, variable selection, multiple testing, shrinkage priors and other relevant areas in statistics \citep{Wenhua2009}. Even though Bayes' rule is clear on how to perform inference for the multivariate mean $b=(b_1,..., b_K)$, since $p(b | y) \propto p(y|b)p(b)$, the main issue lies in how to specify $p(b)$ such that optimality is reached with respect to some criteria that has been chosen beforehand \citep{armagan2013conditions}.

==> tikz/sr2_new.tex <==
\begin{tikzpicture}[node distance=3cm, auto, thick]

    % Define more fitting colors for Fantastic Mr. Fox
    \definecolor{foxorange}{rgb}{0.92, 0.51, 0.19}   % Warm orange for $R^2$
    \definecolor{foxyellow}{rgb}{0.96, 0.87, 0.39}   % Mustard yellow for $\omega^2$
    \definecolor{foxgreen}{rgb}{0.26, 0.59, 0.28}    % Muted green for $\phi_k$
    \definecolor{foxbrown}{rgb}{0.61, 0.35, 0.19}    % Brown for $\lambda_k^2$
    \definecolor{foxred}{rgb}{0.67, 0.23, 0.12}      % Red for $b_k$

    % Nodes with color for better distinction and tree-like layout
    \node[state, draw=foxorange, fill=foxorange!30, minimum width=1.5cm] (r2) at (0,0) {$R^2$};
    \node[state, draw=foxyellow, fill=foxyellow!30, minimum width=1.5cm, right=of r2] (t2) {$\omega^2$};
    
    % Phi nodes
    \node[state, draw=foxgreen, fill=foxgreen!30, minimum width=1.5cm, right=of t2] (phip) {$\phi_1$};
    \node[vmissing, below=of phip] (dots4) {};
    \node[state, draw=foxgreen, fill=foxgreen!30, minimum width=1.5cm, below=of dots4] (phip1) {$\phi_K$};
    
    % Lambda nodes
    \node[state, draw=foxbrown, fill=foxbrown!30, minimum width=1.5cm, below=of phip1] (lambdap) {$\lambda_1^2$};
    \node[vmissing, below=of lambdap] (dots6) {};
    \node[state, draw=foxbrown, fill=foxbrown!30, minimum width=1.5cm, below=of dots6] (lambdap1) {$\lambda_K^2$};
    
    % Beta nodes
    \node[state, draw=foxred, fill=foxred!30, minimum width=1.5cm, below=of lambdap1] (betap) {$b_1$};
    \node[vmissing, below=of betap] (dots8) {};
    \node[state, draw=foxred, fill=foxred!30, minimum width=1.5cm, below=of dots8] (betap1) {$b_K$};

    % Paths with arrows
    \path[->, thick] (r2) edge (t2);
    \path[->, thick] (t2) edge (phip);
    \path[->, thick] (t2) edge (phip1);
    \path[->, thick] (phip) edge (lambdap);
    \path[->, thick] (phip1) edge (lambdap1);
    \path[->, thick] (lambdap) edge (betap);
    \path[->, thick] (lambdap1) edge (betap1);

    % Paths for the dots to indicate continuation
    \path[->, thick] (phip1) edge (dots4);
    \path[->, thick] (lambdap1) edge (dots6);
    \path[->, thick] (betap1) edge (dots8);
    
\end{tikzpicture}



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

